Verified Code Transpilation with LLMs

Domain-specific languages (DSLs) are integral to various software workflows. Such languages offer domain-specific optimizations and abstractions that improve code readability and maintainability. However, leveraging these languages requires developers to rewrite existing code using the specific DSL's API. While large language models (LLMs) have shown some success in automatic code transpilation, none of them provide any functional correctness guarantees on the transpiled code. Another approach for automating this task is verified lifting, which relies on program synthesis to find programs in the target language that are functionally equivalent to the source language program. While several verified lifting tools have been developed for various application domains, they are specialized for specific source-target languages or require significant expertise in domain knowledge to make the search efficient. In this paper, leveraging recent advances in LLMs, we propose an LLM-based approach (LLMLift) to building verified lifting tools. We use the LLM's capabilities to reason about programs to translate a given program into its corresponding equivalent in the target language. Additionally, we use LLMs to generate proofs for functional equivalence. We develop lifting-based compilers for {\em four different} DSLs targeting different application domains. Our approach not only outperforms previous symbolic-based tools in both the number of benchmarks transpiled and transpilation time, but also requires significantly less effort to build.

==> Figures/promp_struc.tex <==
% \begin{figure}[t]
% % \begin{subfigure}{0.4\textwidth}
%     \centering
%     \includegraphics[scale=0.5, trim=0cm 0cm 0cm 0cm]{Figures/prompt_structure.png}
%     \caption{Prompt Structure}
%     \label{fig:prompt_struc}
% \end{figure}


==> Figures/prompt.tex <==
\begin{figure}[t]
% \begin{subfigure}{0.3\textwidth}
%     \centering
%     \includegraphics[scale=0.8, trim=6cm 3cm 6cm 0cm]{Figures/prompt_ps.pdf}
%     \caption{PS guessing prompt}
%     \label{fig:prompt_ps}
% \end{subfigure}
\begin{subfigure}{\textwidth}
 \centering
    \includegraphics[scale=0.5, trim=0cm 0cm 0cm 0cm]{Figures/prompt_structure.png}
    \caption{Prompt Structure}
    \label{fig:prompt_struc}
\end{subfigure}
\end{figure}
% \begin{figure}
%     \centering
%     \includegraphics[scale=0.15, trim=0cm 0cm 0cm 0cm]{Figures/prompt_inv.jpg}
%     \caption{Invariant guessing prompt}
%     \label{fig:prompt_inv}
% % \end{subfigure}
% \end{figure}

